Neurosymbolic AI for Reasoning on Biomedical Knowledge Graphs

Biomedical datasets are often modeled as knowledge graphs (KGs) because they capture the multi-relational, heterogeneous, and dynamic natures of biomedical systems. KG completion (KGC), can, therefore, help researchers make predictions to inform tasks like drug repositioning. While previous approaches for KGC were either rule-based or embedding-based, hybrid approaches based on neurosymbolic artificial intelligence are becoming more popular. Many of these methods possess unique characteristics which make them even better suited toward biomedical challenges. Here, we survey such approaches with an emphasis on their utilities and prospective benefits for biomedicine.

==> figures/taxonomy/4A_taxonomy.tex <==
\begin{forest}
    mytree,
    [,phantom
        [\textbf{Logically-Informed Embedding Approaches} (\ref{subsection:fusion})
            [{\textbf{Modular, Two-Step Approaches}\\[0.5em]
            (\textsc{Neuro:Symbolic $\rightarrow$ Neuro})\\[0.5em]
                \textbullet \ Walking RDF and OWL \cite{alshahrani2017neuro, agibetov2018fast}\\
            }]
            
        ]
    ]
    
\end{forest}


==> figures/taxonomy/4B_taxonomy.tex <==
\begin{forest}
    mytree,
    [,phantom
        [\textbf{KG Embeddings and Deep Learning with Logical Constraints} (\ref{subsection:logical_constraints})
            [{\textbf{Logical Constraints on}\\\textbf{the Embedding Space}\\[0.5em]
            (\textsc{Neuro[Symbolic]})\\[0.5em]
                \textbullet \ R2N \cite{marra2021learning}
            }]
            [{\textbf{Learning Representative}\\\textbf{Logic Embeddings}\\[0.5em]
            (\textsc{Neuro}\textsubscript{\textsc{Symbolic}})\\[0.5em]
                \textbullet \ QLogicE \cite{chen2022qlogice}\\
                \textbullet \ Graph Query \\ \; Embeddings \cite{hamilton2018embedding}
            }]
        ]
    ]
\end{forest}


==> figures/taxonomy/4C_taxonomy.tex <==
\begin{forest}
    mytree,
    [,phantom
        [\textbf{Learning Rules for Graph Reasoning} (\ref{subsection:learning_rules})
            [{\textbf{Iterative, EM Algorithm Methods}\\[0.5em]
            (\textsc{Neuro;Symbolic})\\[0.5em]
                \textbullet \ RNNLogic \cite{qu2020rnnlogic}},l sep+=20pt,
                [{\textbf{Learning Rule Weights}\\[0.5em]
                    \textbullet \ BioGRER \cite{zhao2020biomedical} 
                },
                edge path={
                  \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor) -- +(0,-20pt) -| (.child anchor)\forestoption{edge label};
                }]
            ]
            [{\textbf{New Rules: Bridging the Discrete}\\\textbf{and Continuous Spaces}\\[0.5em]
            (\textsc{Neuro;Symbolic})\\[0.5em]
                \textbullet \ NeuralLP \cite{yang2017differentiable}\\ 
                \textbullet \ DRUM \cite{sadeghian2019drum}\\ 
                \textbullet \ LPRules \cite{dash2021lprules}
            }]
            [{\textbf{Path-Based Rule Learning}\\[0.5em]
            (\textsc{Neuro;Symbolic} /\\
            \textsc{Neuro:Symbolic $\rightarrow$ Neuro})\\[0.5em]
                \textbullet \ PoLo \cite{liu2021neural}\\
                \textbullet \ LPRules \cite{dash2021lprules}\\
                \textbullet \ LNN-MP \cite{sen2021combining}
            }]
        ]
    ]
\end{forest}



==> figures/taxonomy/taxonomy2.tex <==
\begin{forest}
    mytree,
    [,phantom
        [\textbf{Neurosymbolic Methods on Biomedical KGs}
            [{\textbf{Logically-Informed}\\\textbf{Embedding Approaches}\\[0.5em]
                \textbullet \ Walking RDF and OWL\\\cite{alshahrani2017neuro}\\  
                \textbullet \ Walking RDF and OWL\\improvement\\\cite{agibetov2018fast}
            }]
            [{\textbf{KGE with Logical Constraints}\\[0.5em]
                \textbullet \ R2N \cite{marra2021learning}\\
                \textbullet \ QLogicE \cite{chen2022qlogice}\\
                \textbullet \ Graph Query \\ \; Embeddings \cite{hamilton2018embedding}
            }]
            [{\textbf{Rule Learning}\\\textbf{Methods}\\[0.5em]
                    \textbullet \ RNNLogic\\\cite{qu2020rnnlogic}\\
                    \textbullet \ BioGRER\\\cite{zhao2020biomedical}\\
                    \textbullet \ NeuralLP\\\cite{yang2017differentiable}\\ 
                    \textbullet \ DRUM\\\cite{sadeghian2019drum}\\ 
                    \textbullet \ LPRules\\\cite{dash2021lprules}\\
                    \textbullet \ PoLo\\\cite{liu2021neural}\\
                    \textbullet \ LPRules\\\cite{dash2021lprules}\\
                    \textbullet \ LNN-MP\\\cite{sen2021combining}
                }]
        ]
    ]
\end{forest}


